Body-rotation behavior of pedestrians for collision avoidance in passing and cross flow

We observe body-rotation behavior of pedestrians to avoid others when they are moving in congested situations. In such cases, body orientation often differs from walking direction, i.e., pedestrians step sideways. In this paper, we focused on a deviation between body orientation and walking direction during collision avoidance by body rotation for counter-flows in narrow corridors quantitatively. We conducted simple experiments in which two pedestrians passed each other. We found that pedestrians rotated their bodies when the width of the corridor was smaller than the sum of the widths of the two pedestrians. This behavior was explained by analyzing the geometry of two ellipses circumscribing each other in a narrow corridor. Moreover, we developed a preliminary model and succeeded to simulate the deviation between body orientation and walking direction during passing observed in the experiments. Furthermore, we performed a cross-flow experiment, which is much more complex and realistic than the passing experiments and confirmed that body-rotation behavior is also an indispensable factor for complex and realistic scenarios.

==> 13_References.tex <==
\providecommand{\newblock}{}
\begin{thebibliography}{10}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{{\tt #1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\eprint}[2][]{\url{#2}}
% Bibliography created with iopart-num v2.1
% /biblio/bibtex/contrib/iopart-num

\bibitem{Schweitzer2007}
Schweitzer F 2007 {\em {Browning Agents and Active Particles}\/} Springer
  Series in Synergetics (Berlin, Heidelberg: Springer Berlin Heidelberg) ISBN
  978-3-540-73844-2

\bibitem{Helbing2001}
Helbing D 2001 {\em Rev. Mod. Phys.\/} {\bf 73} 1067--1141

\bibitem{Schadschneider2010}
Schadschneider A, Chowdhury D, Nishinari K and Santen L 2010 {\em {Stochastic
  Transport in Complex Systems}\/} (Amsterdam/Oxford: Elsevier) ISBN
  978-0-444-52853-7

\bibitem{Helbing1995}
Helbing D and Moln{\'{a}}r P 1995 {\em Phys. Rev. E\/} {\bf 51} 4282--4286

\bibitem{Helbing2000}
Helbing D, Farkas I and Vicsek T 2000 {\em Nature\/} {\bf 407} 487--490

\bibitem{Burstedde2001}
Burstedde C, Klauck K, Schadschneider A and Zittartz J 2001 {\em Physica A\/} {\bf 295} 507--525 
  
\bibitem{Seyfried2005}
Seyfried A, Steffen B, Klingsch W and Boltes M 2005 {\em J. Stat. Mech. Theory
  Exp.\/} {\bf 2005} P10002--P10002 

\bibitem{Jelic2012a}
Jeli{\'{c}} A, Appert-Rolland C, Lemercier S and Pettr{\'{e}} J 2012 {\em Phys.
  Rev. E\/} {\bf 85} 036111 

\bibitem{Hoogendoorn2005}
Hoogendoorn S and Daamen W 2005 {\em Traffic Granular Flow '03\/} (Springer-Verlag Berlin Heidelberg) 373--382

\bibitem{Kretz2006a}
Kretz T, Gr{\"{u}}nebohm A, Kaufman M, Mazur F, Schreckenberg M, Grunebohm A,
  Kaufman M, Mazur F and Schreckenberg M 2006 {\em J. Stat. Mech. Exp.\/} {\bf
  10001} P10001 

\bibitem{Zhang2012a}
Zhang J, Klingsch W, Schadschneider A and Seyfried A 2012 {\em J. Stat. Mech.
  Theory Exp.\/} {\bf 2012} P02002 

\bibitem{Feliciani2016pre}
Feliciani C and Nishinari K 2016 {\em Phys. Rev. E\/} {\bf 94} 032304

\bibitem{Hoogendoorn2005TransSci}
Hoogendoorn S~P and Daamen W 2005 {\em Transp. Sci.\/} {\bf 39} 147--159 

\bibitem{Kretz2006b}
Kretz T, Gr{\"{u}}nebohm A and Schreckenberg M 2006 {\em J. Stat. Mech. Theory
  Exp.\/} {\bf 2006} P10014--P10014 

\bibitem{Seyfried2009}
Seyfried A, Passon O, Steffen B, Boltes M, Rupprecht T and Klingsch W 2009 {\em
  Transp. Sci.\/} {\bf 43} 395--406 

\bibitem{Seyfried2006}
Seyfried A, Steffen B and Lippert T 2006 {\em Physica A\/}
  {\bf 368} 232--238 

\bibitem{Parisi2009}
Parisi D~R, Gilman M and Moldovan H 2009 {\em Physica A\/}
  {\bf 388} 3600--3608 

\bibitem{Kirchner2003a}
Kirchner A, Kl{\"{u}}pfel H, Nishinari K, Schadschneider A and Schreckenberg M
  2003 {\em Physica A\/} {\bf 324} 689--697 

\bibitem{Kirchner2003b}
Kirchner A, Nishinari K and Schadschneider A 2003 {\em Phys. Rev. E\/} {\bf 67}
  056122 

\bibitem{Yanagisawa2009}
Yanagisawa D, Kimura A, Tomoeda A, Nishi R, Suma Y, Ohtsuka K and Nishinari K
  2009 {\em Phys. Rev. E\/} {\bf 80} 036110 

\bibitem{Henein2007}
Henein C~M and White T 2007 {\em Physica A\/} {\bf 373}
  694--712 

\bibitem{Henein2010}
Henein C~M and White T 2010 {\em Physica A\/} {\bf 389}
  4636--4653 

\bibitem{Suma2012}
Suma Y, Yanagisawa D and Nishinari K 2012 {\em Physica A\/}
  {\bf 391} 248--263 

\bibitem{Nowak2012}
Nowak S and Schadschneider A 2012 {\em Phys. Rev. E\/} {\bf 85} 066128 

\bibitem{Weng2006}
Weng W~G, Chen T, Yuan H~Y and Fan W~C 2006 {\em Phys. Rev. E\/} {\bf 74}
  036102 

\bibitem{Jiang2007}
Jiang R and Wu Q~S 2007 {\em Physica A\/} {\bf 373}
  683--693 

\bibitem{Hrabak2016}
Hrab{\'{a}}k P and Buk{\'{a}}{\v{c}}ek M 2016 {\em Lecture Notes in Computer Science
  (Parallel Process. Appl. Math.)\/} {\bf 3911} 507--516

\bibitem{Bandini2009}
Bandini S, Manzoni S and Vizzari G 2009 {\em J. Artif. Soc. Soc. Simul.\/} {\bf
  12} 4

\bibitem{Bandini2015}
Bandini S, Crociani L and Vizzari G 2015  {\em Ambient Assisted Living\/} (Springer International Publishing) 11--21 ISBN
  978-3-319-18374-9

\bibitem{Yanagisawa2012}
Yanagisawa D, Tomoeda A and Nishinari K 2012 {\em Phys. Rev. E\/} {\bf 85}
  016111

\bibitem{Jelic2012b}
Jeli{\'{c}} A, Appert-Rolland C, Lemercier S and Pettr{\'{e}} J 2012 {\em Phys.
  Rev. E\/} {\bf 86} 046111

\bibitem{Sivers2015}
von Sivers I and K{\"{o}}ster G 2015 {\em Transp. Res. Part B\/} {\bf
  74} 104--117

\bibitem{Liu2016b}
Liu X, Song W, Fu L, Lv W and Fang Z 2016 {\em Phys. Lett. A\/} {\bf 380}
  1526--1534

\bibitem{Ezaki2016cd}
Ezaki T, Ohtsuka K, Chraibi M, Boltes M, Yanagisawa D, Seyfried A,
  Schadschneider A and Nishinari K 2016 {\em Collect. Dyn.\/} {\bf 1} A4
  
\bibitem{Ezaki2012a}
Ezaki T, Yanagisawa D, Ohtsuka K and Nishinari K 2012 {\em Physica A\/} {\bf 391} 291--299

\bibitem{Ezaki2015tgf}
Ezaki T, Ohtsuka K, Yanagisawa D and Nishinari K 2015 {\em Traffic Granular Flow '13\/} ed Chraibi M,
  Boltes M, Schadschneider A and Seyfried A (Cham: Springer International
  Publishing) 227--231 ISBN 978-3-319-10628-1

\bibitem{Blue2001}
Blue V~J and Adler J~L 2001 {\em Transp. Res. Part B\/} {\bf 35}
  293--312

\bibitem{Feliciani2016PhysicaA}
Feliciani C and Nishinari K 2016 {\em Physica A\/} {\bf
  451} 135--148

\bibitem{Yanagisawa2016cd}
Yanagisawa D 2016 {\em Collect. Dyn.\/} {\bf 1} A8

\bibitem{Fruin1971}
Fruin J~J 1971 {\em {Pedestrian planning and design}\/} (Metropolitan
  Association of Urban Designers and Environmental Planners)

\bibitem{Pauls2004}
Pauls J 2004 {Suggestions on evacuation models and research questions} {\em
  Proc. Third Int. Symp. Hum. Behav. Fire\/} 2001 ed Shields T~J (London:
  Interscience)

\bibitem{Was2006}
W{\c{a}}s J, Gudowski B and Matuszyk P~J 2006 {\em Lecture Notes in Computer Science
  (Cellular Automata)\/} {\bf 4173} 492--501

\bibitem{Chraibi2010}
Chraibi M, Seyfried A and Schadschneider A 2010 {\em Phys. Rev. E\/} {\bf 82}
  046111

\bibitem{Moussaid2009}
Moussaid M, Helbing D, Garnier S, Johansson A, Combe M and Theraulaz G 2009
  {\em Proc. R. Soc. B Biol. Sci.\/} {\bf 276} 2755--2762

\bibitem{Imai2001}
Imai T, Moore S~T, Raphan T and Cohen B 2001 {\em Exp. Brain Res.\/} {\bf 136}
  1--18

\bibitem{Gorrini2014b}
Gorrini A, Shimura K, Bandini S, Ohtsuka K and Nishinari K 2014 {\em Transp.
  Res. Rec. J. Transp. Res. Board\/} {\bf 2421} 57--63

\bibitem{Olivier2013}
Olivier A~H, Marin A, Cr{\'{e}}tual A, Berthoz A and Pettr{\'{e}} J 2013 {\em
  Gait Posture\/} {\bf 38} 751--756

\bibitem{Daamen2014}
Daamen W, Hoogendoorn S, Campanella M and Versluis D 2014 {\em Pedestrian and Evacuation Dynamics 2012\/}  1305--1313 ISSN 0012-3692

\bibitem{Huber2014}
Huber M, Su Y~H, Kr{\"{u}}ger M, Faschian K, Glasauer S and Hermsd{\"{o}}rfer J
  2014 {\em PLoS One\/} {\bf 9} e89589

\bibitem{Parisi2016}
Parisi D~R, Negri P~A and Bruno L 2016 {\em Phys. Rev. E\/} {\bf 94} 022318

\bibitem{Zanlungo2012}
Zanlungo F, Ikeda T and Kanda T 2012 {\em PLoS One\/} {\bf 7} e50720

\bibitem{Feliciani2016ped}
Feliciani C and Nishinari K 2016 {\em Pedestrian and Evacuation Dynamics 2016\/} ed Song W, Ma J
  and Fu L (Hefei: University of Science and Technology of China Press) 76--83 ISBN 978-7-312-04077-1 (\textit{Preprint} \eprint{arXiv:1610.07185})

\bibitem{sizeJPN2004-2006}
{\em {Report on size-JPN 2004-2006}\/} 2007 (Ministry of Economy, Trade and
  Industry in Japan) (in Japanese)
  \urlprefix\url{http://warp.da.ndl.go.jp/info:ndljp/pid/281883/www.meti.go.jp/press/\\20071001007/20071001007.html}

\bibitem{Zheng2007}
Zheng X and Palffy-Muhoray P 2007 {\em Phys. Rev. E\/} {\bf 75} 061709

\bibitem{Chraibi2012rg}
Chraibi M 2012 Distance of closest approach of ellipse and line segment {\em ResearchGate\/}
  \urlprefix\url{https://www.researchgate.net/publication/\\306107046{\_}Distance{\_}of{\_}closest{\_}approach{\_}of{\_}ellipse{\_}and{\_}line{\_}segment}

\end{thebibliography}

